On Context Utilization in Summarization with Large Language Models

Large language models (LLMs) excel in abstractive summarization tasks, delivering fluent and pertinent summaries. Recent advancements have extended their capabilities to handle long-input contexts, exceeding 100k tokens. However, in question answering, language models exhibit uneven utilization of their input context. They tend to favor the initial and final segments, resulting in a U-shaped performance pattern concerning where the answer is located within the input. This bias raises concerns, particularly in summarization where crucial content may be dispersed throughout the source document(s). Besides, in summarization, mapping facts from the source to the summary is not trivial as salient content is usually re-phrased. In this paper, we conduct the first comprehensive study on context utilization and position bias in summarization. Our analysis encompasses 6 LLMs, 10 datasets, and 5 evaluation metrics. We introduce a new evaluation benchmark called MiddleSum on the which we benchmark two alternative inference methods to alleviate position bias: hierarchical summarization and incremental summarization. Our code and data can be found here: https://github.com/ntunlp/MiddleSum.

==> Tables/unused_corr_cr.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]

\resizebox{\textwidth}{!}{
\begin{tabular}{l@{\hspace{10pt}}l@{\hspace{10pt}}ccccc|ccccc|c}

\toprule 

\textbf{Model}                        
& \textbf{Metric} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{CNN/DM}}}
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{XSum}}}
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{Reddit-TIFU}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{SAMSum}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{Arxiv}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{PubMed}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{GovReport}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{SummScreen}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{Multi-News}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{Multi-XScience}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{AVERAGE}}} \\

\midrule 

\multirow{5}{*}{\textbf{FLAN-UL2}}
& Mean-R & \grlow{-0.233} & \grlow{-0.115} & \grlow{-0.157} & \grlow{-0.188} & \grhigh{0.129} & \grhigh{0.063} & \grlow{-0.053} & \grhigh{0.087} & \grlow{-0.015} & \grlow{-0.226} & \textbf{\grlow{-0.075}} \\
& BS     & \grlow{-0.209} & \grlow{-0.132} & \grlow{-0.058} & \grlow{-0.151} & \grhigh{0.200} & \grhigh{0.013} & \grlow{-0.127} & \grhigh{0.318} & \grlow{-0.111} & \grlow{-0.260} &  \textbf{\grlow{-0.052}} \\
& SUPERT & \\ 
& BaS-f & \\ 
 & GPT-3.5 &   \\


\cdashline{1-13}
% \midrule 

\multirow{5}{*}{\textbf{LLAMA-2-7B}}
& Mean-R & \grlow{-0.376} & \grlow{-0.027} & \grlow{-0.352} & \grlow{-0.409} & \grlow{-0.094} & \grlow{-0.296} & \grlow{-0.163} & \grlow{-0.176} & \grlow{-0.255} & \grlow{-0.416} & \textbf{\grlow{-0.256}} \\
& BS     & \grlow{-0.250} & \grlow{-0.024} & \grlow{-0.267} & \grlow{-0.355} & \grhigh{0.085} & \grlow{-0.200} & \grlow{-0.197} & \grhigh{0.195} & \grlow{-0.230} & \grlow{-0.393} & \textbf{\grlow{-0.164}} \\
& SUPERT & \\ 
& BaS-f & \\ 
 & GPT-3.5 & \\

\cdashline{1-13}

\multirow{5}{*}{\textbf{LLAMA-2-13B}}
& Mean-R & \grlow{-0.317} & \grlow{-0.105} & \grlow{-0.361} & \grlow{-0.371} & \grlow{-0.146} & \grlow{-0.255} & \grlow{-0.219} & \grlow{-0.239} & \grlow{-0.197} & \grlow{-0.428} & \textbf{\grlow{-0.264}} \\
& BS     & \grlow{-0.203} & \grlow{-0.080} & \grlow{-0.258} & \grlow{-0.307} & \grhigh{0.039} & \grlow{-0.120} & \grlow{-0.193} & \grhigh{0.170} & \grlow{-0.240} & \grlow{-0.365} & \textbf{\grlow{-0.156}} \\
& SUPERT & \\ 
& BaS-f &  \\ 
 & GPT-3.5 & \\

\cdashline{1-13}

\multirow{5}{*}{\textbf{XGen-7B}}                 
& Mean-R & \grlow{-0.297} & \grlow{-0.064} & \grlow{-0.385} & \grlow{-0.328} & \grlow{-0.156} & \grlow{-0.268}  & \grlow{-0.355} & \grlow{-0.327} & \grlow{-0.189} & \grlow{-0.411} & \textbf{\grlow{-0.278}} \\ 
& BS     & \grlow{-0.206} & \grlow{-0.068} & \grlow{-0.272} & \grlow{-0.289} & \grhigh{0.004} & \grlow{-0.128} & \grlow{-0.289} & \grhigh{0.080} & \grlow{-0.267} & \grlow{-0.351} & \textbf{\grlow{-0.179}} \\
& SUPERT &  \\ 
& BaS-f &  \\ 
 & GPT-3.5 &  \\

\bottomrule

\end{tabular}
}
\vspace{-0.5em}
\caption{\small Spearman correlation coefficient between each LLM's metric, and the compression ratio (where source and target lengths are measured in tokens). Mean-R is the arithmetic average of \{ROUGE-1, ROUGE-2, ROUGE-L-Sum\}, BS is BERTScore, BaS-f is BARTScore-faithfulness.}
\vspace{-1.0em}
\label{corr_cr}
\end{table*}

==> Tables/unused_corr_pred_length.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]

\resizebox{\textwidth}{!}{
\begin{tabular}{l@{\hspace{10pt}}l@{\hspace{10pt}}ccccccccccccc}

\toprule 

\textbf{Model}                        
& \textbf{Metric} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{CNN/DM}}}
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{XSum}}}
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{Reddit-TIFU}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{SAMSum}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{Arxiv}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{PubMed}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{GovReport}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{SummScreen}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{QMSum}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{Multi-News}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{Multi-XScience}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{AquaMuse}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{AVERAGE}}} \\

\midrule 

\multirow{5}{*}{\textbf{FLAN-UL2}}
& Mean-R & \grhigh{0.219} & \grlow{-0.114} & \grhigh{0.071} & \grlow{-0.093} & \grhigh{0.760} & \grhigh{0.629} & \grhigh{0.836} & \grhigh{0.430} & \grhigh{0.458} & \grhigh{0.830} & \grhigh{0.702} & \grhigh{0.645} & \textbf{\grhigh{0.448}} \\ 
& BS     & \grlow{-0.007} & \grlow{-0.184} & \grlow{-0.125} & \grlow{-0.190} & \grhigh{0.366} & \grhigh{0.228} & \grhigh{0.380} & \grlow{-0.157} & \grlow{-0.020} & \grhigh{0.337} & \grhigh{0.310} & \grhigh{0.307} & \textbf{\grhigh{0.104}} \\
& SUPERT & \grhigh{0.603} & \grhigh{0.097} & \grhigh{0.480} & \grhigh{0.021} & \grhigh{0.403} & \grhigh{0.411} & \grhigh{0.430} & \grhigh{0.483} & \grhigh{0.429} & \grhigh{0.629} & \grhigh{0.686} & \grhigh{0.452} & \textbf{\grhigh{0.427}} \\ 
& BaS-f & \grhigh{0.522} & \grhigh{0.077} & \grhigh{0.592} & \grhigh{0.213} & \grhigh{0.612} & \grhigh{0.535} & \grhigh{0.472} & \grhigh{0.272} & \grhigh{0.312} & \grhigh{0.467} & \grhigh{0.763} & \grhigh{0.590} & \textbf{\grhigh{0.452}} \\
& GPT-3.5 & \grhigh{0.397} & \grhigh{0.231} & \grhigh{0.693} & \grhigh{0.273} & \grhigh{0.727} & \grhigh{0.678} & \grhigh{0.395} & \grhigh{0.523} & \grhigh{0.525} & \grhigh{0.874} & \grhigh{0.912} & \grhigh{0.846} & \textbf{\grhigh{0.590}} \\

\cdashline{1-14}
% \midrule 

\multirow{5}{*}{\textbf{LLAMA-2-7B}}
& Mean-R & \grlow{-0.033} & \grlow{-0.073} & \grlow{-0.034} & \grlow{-0.243} & \grlow{-0.054} & \grlow{-0.359} & \grhigh{0.233} & \grhigh{0.094} & \grhigh{0.053} & \grlow{-0.042} & \grhigh{0.108} & \grhigh{0.084} & \textbf{\grlow{-0.022}} \\ 
& BS     & \grlow{-0.056} & \grlow{-0.221} & \grlow{-0.108} & \grlow{-0.376} & \grlow{-0.144} & \grlow{-0.417} & \grlow{-0.187} & \grlow{-0.152} & \grlow{-0.192} & \grlow{-0.183} & \grlow{-0.100} & \grhigh{0.028} & \textbf{\grlow{-0.176}} \\
& SUPERT & \grhigh{0.062} & \grhigh{0.002} & \grhigh{0.005} & \grlow{-0.257} & \grhigh{0.139} & \grlow{-0.152} & \grhigh{0.023} & \grlow{-0.004} & \grhigh{0.215} & \grhigh{0.029} & \grhigh{0.057} & \grhigh{0.142} & \textbf{\grhigh{0.022}} \\ 
& BaS-f & \grhigh{0.018} & \grlow{-0.134} & \grhigh{0.034} & \grlow{-0.130} & \grlow{-0.102} & \grlow{-0.377} & \grlow{-0.009} & \grhigh{0.134} & \grhigh{0.183} & \grlow{-0.096} & \grhigh{0.312} & \grhigh{0.035} & \textbf{\grlow{-0.011}} \\
& GPT-3.5 & \grhigh{0.071} & \grhigh{0.007} & \grhigh{0.055} & \grlow{-0.068} & \grhigh{0.352} & \grlow{-0.152} & \grhigh{0.253} & \grhigh{0.328} & \grhigh{0.509} & \grhigh{0.259} & \grhigh{0.256} & \grhigh{0.229} & \textbf{\grhigh{0.175}} \\

\cdashline{1-14}

\multirow{5}{*}{\textbf{LLAMA-2-13B}}
& Mean-R & \grlow{-0.054} & \grlow{-0.090} & \grlow{-0.066} & \grlow{-0.152} & \grhigh{0.036} & \grhigh{0.142} & \grhigh{0.463} & \grlow{-0.057} & \grlow{-0.046} & \grhigh{0.045} & \grhigh{0.111} & \grhigh{0.132} & \textbf{\grhigh{0.039}} \\ 
& BS     & \grlow{-0.097} & \grlow{-0.262} & \grlow{-0.177} & \grlow{-0.251} & \grlow{-0.146} & \grhigh{0.003} & \grlow{-0.181} & \grlow{-0.192} & \grlow{-0.244} & \grlow{-0.226} & \grlow{-0.016} & \grhigh{0.053} & \textbf{\grlow{-0.145}} \\
& SUPERT & \grhigh{0.040} & \grhigh{0.036} & \grhigh{0.019} & \grlow{-0.070} & \grhigh{0.157} & \grhigh{0.169} & \grlow{-0.064} & \grhigh{0.001} & \grhigh{0.237} & \grhigh{0.054} & \grhigh{0.070} & \grhigh{0.143} & \textbf{\grhigh{0.066}} \\ 
& BaS-f & \grhigh{0.005} & \grlow{-0.123} & \grhigh{0.044} & \grhigh{0.062} & \grhigh{0.067} & \grhigh{0.131} & \grlow{-0.021} & \grhigh{0.021} & \grhigh{0.233} & \grlow{-0.243} & \grhigh{0.291} & \grhigh{0.112} & \textbf{\grhigh{0.048}} \\
& GPT-3.5 & \grlow{-0.050} & \grhigh{0.158} & \grlow{-0.110} & \grlow{-0.134} & \grhigh{0.382} & \grhigh{0.113} & \grhigh{0.552} & \grlow{-0.064} & \grhigh{0.352} & \grhigh{0.152} & \grhigh{0.299} & \grhigh{0.218} & \textbf{\grhigh{0.156}} \\

\cdashline{1-14}

\multirow{5}{*}{\textbf{XGen-7B}}                 
& Mean-R & \grlow{-0.167} & \grlow{-0.200} & \grlow{-0.135} & \grlow{-0.274} & \grlow{-0.329} & \grlow{-0.141} & \grhigh{0.275} & \grlow{-0.231} & \grlow{-0.407} & \grhigh{0.158} & \grhigh{0.004} & \grlow{-0.020} & \textbf{\grlow{-0.122}} \\ 
& BS     & \grlow{-0.225} & \grlow{-0.311} & \grlow{-0.299} & \grlow{-0.417} & \grlow{-0.483} & \grlow{-0.351} & \grlow{-0.222} & \grlow{-0.576} & \grlow{-0.769} & \grlow{-0.336} & \grlow{-0.254} & \grlow{-0.153} & \textbf{\grlow{-0.366}} \\
& SUPERT & \grhigh{0.338} & \grhigh{0.195} & \grhigh{0.347} & \grlow{-0.081} & \grhigh{0.271} & \grhigh{0.263} & \grhigh{0.223} & \grhigh{0.235} & \grhigh{0.214} & \grhigh{0.272} & \grhigh{0.328} & \grhigh{0.178} & \textbf{\grhigh{0.232}} \\ 
& BaS-f & \grhigh{0.345} & \grhigh{0.321} & \grhigh{0.569} & \grhigh{0.446} & \grhigh{0.539} & \grhigh{0.412} & \grhigh{0.423} & \grhigh{0.458} & \grhigh{0.719} & \grhigh{0.342} & \grhigh{0.558} & \grhigh{0.268} & \textbf{\grhigh{0.450}} \\
& GPT-3.5 & \grhigh{0.307} & \grhigh{0.083} & \grhigh{0.042} & \grlow{-0.001} & \grhigh{0.624} & \grhigh{0.616} & \grhigh{0.572} & \grhigh{0.658} & \grhigh{0.645} & \grhigh{0.606} & \grhigh{0.473} & \grhigh{0.281} & \textbf{\grhigh{0.409}} \\

\bottomrule

\end{tabular}
}
\caption{\small Spearman correlation coefficient between each LLM's metric, and the generated summary length (measured in terms of tokens).}
\label{corr_pred_length}
\end{table*}

==> Tables/unused_corr_source_length.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]

\resizebox{\textwidth}{!}{
\begin{tabular}{l@{\hspace{10pt}}l@{\hspace{10pt}}ccccc|ccccc|c}

\toprule 

\textbf{Model}                        
& \textbf{Metric} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{CNN/DM}}}
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{XSum}}}
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{Reddit-TIFU}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{SAMSum}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{Multi-XScience}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{Arxiv}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{PubMed}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{GovReport}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{SummScreen}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{Multi-News}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{AVERAGE}}} \\

\midrule 

\multirow{5}{*}{\textbf{FLAN-UL2}}
& Mean-R & \grlow{-0.108} & \grlow{-0.168} & \grlow{-0.055} & \grlow{-0.242} & \grlow{-0.415} & \grlow{-0.093} & \grlow{-0.174} & \grlow{-0.187} & \grlow{-0.192} & \grlow{-0.120} & \textbf{\grlow{-0.151}} \\
& BS     & \grlow{-0.204} & \grlow{-0.210} & \grlow{-0.083} & \grlow{-0.274} & \grlow{-0.537} & \grlow{-0.101} & \grlow{-0.303} & \grlow{-0.196} & \grlow{-0.092} & \grlow{-0.229} & \textbf{\grlow{-0.223}} \\
& SUPERT & \grlow{-0.018} & \grlow{-0.011} & \grlow{-0.273}  & \grlow{-0.338} & \grlow{-0.578} & \grlow{-0.031} & \grhigh{0.009} & \grlow{-0.066} & \grlow{-0.089} & \grlow{-0.164} & \textbf{\grlow{-0.156}} \\ 
& BaS-f & \grlow{-0.014} & \grhigh{0.100} & \grhigh{0.046} & \grlow{-0.020} & \grlow{-0.555} & \grlow{-0.036} & \grlow{-0.075} & \grlow{-0.099} & \grhigh{0.022} & \grlow{-0.352} & \textbf{\grlow{-0.098}} \\ 
& GPT-3.5 & \\

\cdashline{1-13}
% \midrule 

\multirow{5}{*}{\textbf{LLAMA-2-7B}}
& Mean-R & \grlow{-0.177}  & \grlow{-0.004} & \grhigh{0.126} & \grlow{-0.149} & \grlow{-0.056} & \grhigh{0.057} & \grlow{-0.186} & \grlow{-0.242} & \grlow{-0.011}  & \grlow{-0.192} & \textbf{\grlow{-0.083}} \\
& BS     & \grlow{-0.221} & \grlow{-0.066} & \grlow{-0.016} & \grlow{-0.272} & \grlow{-0.470} & \grlow{-0.079} & \grlow{-0.287} & \grlow{-0.212} & \grlow{-0.144} & \grlow{-0.295} & \textbf{\grlow{-0.206}} \\
& SUPERT & \grlow{-0.373} & \grlow{-0.355} & \grlow{-0.548} & \grlow{-0.465} & \grlow{-0.754} & \grlow{-0.125} & \grlow{-0.353} & \grlow{-0.040} & \grlow{-0.058} & \grlow{-0.317} & \textbf{\grlow{-0.307}} \\ 
& BaS-f & \grlow{-0.253} & \grlow{-0.308} & \grlow{-0.096} & \grlow{-0.154} & \grlow{-0.479} & \grlow{-0.112} & \grlow{-0.445} & \grlow{-0.022} & \grlow{-0.211} & \grlow{-0.568} & \textbf{\grlow{-0.265}} \\ 
& GPT-3.5 & \\

\cdashline{1-13}

\multirow{5}{*}{\textbf{LLAMA-2-13B}}
& Mean-R & \grlow{-0.121} & \grlow{-0.092} & \grhigh{0.080} & \grlow{-0.121} & \grlow{-0.071} & \grlow{-0.017} & \grlow{-0.099} & \grlow{-0.263} & \grhigh{0.019} & \grlow{-0.183} & \textbf{\grlow{-0.087}} \\
& BS     & \grlow{-0.189} & \grlow{-0.123} & \grlow{-0.021} & \grlow{-0.211} & \grlow{-0.452} & \grlow{-0.164} & \grlow{-0.275} & \grlow{-0.205} & \grlow{-0.111} & \grlow{-0.322} & \textbf{\grlow{-0.207}} \\
& SUPERT & \grlow{-0.356} & \grlow{-0.329} & \grlow{-0.555} & \grlow{-0.447} & \grlow{-0.772} & \grlow{0.000} & \grlow{-0.037} & \grlow{-0.046} & \grlow{-0.060} & \grlow{-0.276} & \textbf{\grlow{-0.288}} \\ 
& BaS-f & \grlow{-0.215} & \grlow{-0.262} & \grlow{-0.102} & \grhigh{0.072} & \grlow{-0.542} & \grhigh{0.000} & \grlow{-0.221} & \grlow{-0.038} & \grlow{-0.094} &  \grlow{-0.590} & \textbf{\grlow{-0.199}} \\ 
& GPT-3.5 &  \\

\cdashline{1-13}

\multirow{5}{*}{\textbf{XGen-7B}}                 
& Mean-R & \grlow{-0.116} & \grlow{-0.042} & \grhigh{0.069} & \grlow{-0.130} & \grlow{-0.007} & \grlow{-0.002} & \grhigh{0.080} & \grlow{-0.370} & \grlow{-0.001} & \grlow{-0.192} & \textbf{\grlow{-0.071}} \\ 
& BS     & \grlow{-0.194} & \grlow{-0.121} & \grlow{-0.028} & \grlow{-0.234} & \grlow{-0.411} & \grlow{-0.084} & \grlow{-0.111} & \grlow{-0.350} & \grlow{-0.083} & \grlow{-0.344} & \textbf{\grlow{-0.196}} \\
& SUPERT & \grlow{-0.214} & \grlow{-0.367} & \grlow{-0.492} & \grlow{-0.466} & \grlow{-0.721} & \grlow{-0.458} & \grlow{-0.475} & \grlow{-0.364} & \grlow{-0.175} & \grlow{-0.254} & \textbf{\grlow{-0.399}} \\ 
& BaS-f & \grlow{-0.151} & \grlow{-0.192} & \grlow{-0.061} & \grhigh{0.102} & \grlow{-0.397} & \grlow{-0.434} & \grlow{-0.460} & \grlow{-0.265} & \grlow{-0.080} & \grlow{-0.360} & \textbf{\grlow{-0.230}} \\ 
& GPT-3.5 &  \\

\bottomrule

\end{tabular}
}
\caption{\small Spearman correlation coefficient between each LLM's metric, and the source length (measured in terms of tokens).}
\label{corr_source_length}
\end{table*}

==> Tables/unused_corr_target_length.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]

\resizebox{\textwidth}{!}{
\begin{tabular}{l@{\hspace{10pt}}l@{\hspace{10pt}}ccccccccccccc}

\toprule 

\textbf{Model}                        
& \textbf{Metric} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{CNN/DM}}}
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{XSum}}}
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{Reddit-TIFU}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{SAMSum}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{Arxiv}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{PubMed}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{GovReport}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{SummScreen}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{QMSum}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{Multi-News}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{Multi-XScience}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{AquaMuse}}} 
& \multicolumn{1}{c}{\rotatebox[origin=l]{60}{\textbf{AVERAGE}}} \\

\midrule 

\multirow{5}{*}{\textbf{FLAN-UL2}}
& Mean-R & \grhigh{0.200} & \grlow{-0.130} & \grhigh{0.124} & \grlow{-0.125} & \grlow{-0.386} & \grlow{-0.333} & \grlow{-0.304} & \grlow{-0.222} & \grlow{-0.065} & \grlow{-0.252} & \grlow{-0.270} & \grlow{-0.309} & \textbf{\grlow{-0.173}} \\
& BS     & \grhigh{0.028} & \grlow{-0.205} & \grlow{-0.021} & \grlow{-0.216} & \grlow{-0.498} & \grlow{-0.469} & \grlow{-0.126} & \grlow{-0.407} & \grlow{-0.187} & \grlow{-0.332} & \grlow{-0.380} & \grlow{-0.269} & \textbf{\grlow{-0.257}} \\
% & MS     & \grhigh{0.114} & \grlow{-0.161} & \grlow{-0.015} & \grlow{-0.114} & \grlow{-0.368} & \grlow{-0.269} & \grlow{-0.060} & \grlow{-0.288} & \grlow{-0.128} & \grlow{-0.225}  & \grlow{-0.336} & \grlow{-0.219} & \grlow{-0.172} \\
% & BaS    & \grhigh{0.184} & \grlow{-0.181} & \grhigh{0.280} & \grlow{-0.118} & \grlow{-0.009} & \grhigh{0.120} & \grlow{-0.098} & \grhigh{0.067} & \grhigh{0.206} & \grlow{-0.086} & \grhigh{0.068} & \grlow{-0.063} & \grhigh{0.031} \\
& SUPERT & \grhigh{0.230} & \grlow{-0.034} & \grlow{-0.048} & \grlow{-0.173} & \grlow{-0.064} & \grhigh{0.081} & \grlow{-0.033} & \grlow{-0.010} & \grhigh{0.031} & \grlow{-0.237} & \grlow{-0.318} & \grlow{-0.046} & \textbf{\grlow{-0.052}} \\ 
& BaS-f & \grhigh{0.252} & \grhigh{0.010} & \grhigh{0.045} & \grhigh{0.073} & \grlow{-0.055} & \grhigh{0.059} & \grhigh{0.002} & \grlow{-0.006} & \grhigh{0.227} & \grlow{-0.116} & \grlow{-0.314} & \grlow{-0.089} & \textbf{\grhigh{0.007}} \\ 
& GPT-3.5 & \grhigh{0.271} & \grhigh{0.285} & \grlow{-0.136} & \grlow{-0.007} & \grlow{-0.162} & \grhigh{0.017} & \grlow{-0.206} & \grhigh{0.064} & \grhigh{0.201} & \grlow{-0.076} & \grlow{-0.215} & \grhigh{0.067} & \textbf{\grhigh{0.009}} \\

\cdashline{1-14}
% \midrule 

\multirow{5}{*}{\textbf{LLAMA-2-7B}}
& Mean-R & \grhigh{0.339} & \grhigh{0.096} & \grhigh{0.586} & \grhigh{0.254} & \grhigh{0.206} & \grhigh{0.071} & \grlow{-0.231} & \grhigh{0.208} & \grhigh{0.247} & \grhigh{0.044} & \grhigh{0.364} & \grhigh{0.138} & \textbf{\grhigh{0.194}} \\
& BS     & \grhigh{0.071} & \grlow{-0.112} & \grhigh{0.314} & \grhigh{0.008} & \grlow{-0.281} & \grlow{-0.182}  & \grlow{-0.035} & \grlow{-0.294} & \grlow{-0.167} & \grlow{-0.239} & \grlow{-0.157} & \grlow{-0.153} & \textbf{\grlow{-0.102}} \\
% & MS     & \grhigh{0.261} & \grhigh{0.186} & \grhigh{0.681} & \grhigh{0.394} & \grlow{-0.071} & \grlow{-0.047}  & \grlow{-0.042} & \grlow{-0.011} & \grhigh{0.073} & \grlow{-0.107} & \grhigh{0.089} & \grhigh{0.050} & \grhigh{0.121} \\
% & BaS    & \grhigh{0.165} & \grlow{-0.074} & \grhigh{0.418} & \grlow{-0.110} & \grhigh{0.072} & \grhigh{0.086}  & \grlow{-0.016} & \grhigh{0.046} & \grhigh{0.102} & \grlow{-0.134} & \grhigh{0.287} & \grhigh{0.062} & \grhigh{0.075} \\    
& SUPERT & \grlow{-0.034} & \grlow{-0.214} & \grlow{-0.134} & \grlow{-0.274} & \grlow{-0.068} & \grlow{-0.257} & \grlow{-0.028} & \grlow{-0.012} & \grhigh{0.124} & \grlow{-0.289} & \grlow{-0.365} & \grhigh{0.024} & \textbf{\grlow{-0.127}} \\ 
& BaS-f & \grhigh{0.118} & \grlow{-0.106} & \grlow{-0.04} & \grhigh{0.029} & \grlow{-0.052} & \grlow{-0.229} & \grlow{-0.020} & \grlow{-0.028} & \grhigh{0.162} & \grlow{-0.263} & \grlow{-0.237} & \grhigh{0.110} & \textbf{\grlow{-0.046}} \\ 
& GPT-3.5 & \grhigh{0.115} & \grhigh{0.055} & \grlow{-0.092} & \grlow{-0.092} & \grlow{-0.035} & \grlow{-0.185} & \grlow{-0.152} & \grhigh{0.052} & \grhigh{0.066} & \grlow{-0.049} & \grlow{-0.285} & \grhigh{0.194} & \textbf{\grlow{-0.034}} \\

\cdashline{1-14}

\multirow{5}{*}{\textbf{LLAMA-2-13B}}
& Mean-R & \grhigh{0.339} & \grhigh{0.068} & \grhigh{0.549} & \grhigh{0.254} & \grhigh{0.156} & \grhigh{0.141} & \grlow{-0.114} & \grhigh{0.301}  & \grhigh{0.351} & \grlow{-0.058} & \grhigh{0.356} & \grhigh{0.163} & \textbf{\grhigh{0.209}} \\
& BS     & \grhigh{0.059} & \grlow{-0.116} & \grhigh{0.299} & \grhigh{0.060} & \grlow{-0.341} & \grlow{-0.259} & \grlow{-0.020} & \grlow{-0.257} & \grlow{-0.134} & \grlow{-0.288} & \grlow{-0.170} & \grlow{-0.144} & \textbf{\grlow{-0.109}} \\
% & MS     & \grhigh{0.263} & \grhigh{0.160} & \grhigh{0.676} & \grhigh{0.406} & \grlow{-0.158} & \grlow{-0.026} & \grhigh{0.070} & \grhigh{0.066} & \grhigh{0.094} & \grlow{-0.182} & \grhigh{0.033} & \grhigh{0.061} & \grhigh{0.122} \\
% & BaS    & \grhigh{0.156} & \grlow{-0.107} & \grhigh{0.395} & \grlow{-0.035} & \grhigh{0.094} & \grhigh{0.278} & \grhigh{0.025} & \grhigh{0.101} & \grhigh{0.122} & \grlow{-0.114} & \grhigh{0.341} & \grhigh{0.049} & \grhigh{0.109} \\ 
& SUPERT & \grlow{-0.041} & \grlow{-0.196} & \grlow{-0.166} & \grlow{-0.230} & \grlow{-0.021} & \grlow{-0.033} & \grlow{-0.051} & \grlow{-0.079} & \grhigh{0.171} & \grlow{-0.285} & \grlow{-0.380} & \grhigh{0.020} & \textbf{\grlow{-0.108}} \\ 
& BaS-f & \grhigh{0.095} & \grlow{-0.123} & \grlow{-0.008} & \grhigh{0.178} & \grhigh{0.032} & \grlow{-0.033} & \grlow{-0.021} & \grhigh{0.008} & \grhigh{0.177} & \grlow{-0.247} & \grlow{-0.289} & \grhigh{0.129} & \textbf{\grlow{-0.009}} \\ 
& GPT-3.5 & \grhigh{0.069} & \grhigh{0.005} & \grlow{-0.278} & \grlow{-0.060} & \grhigh{0.096} & \grhigh{0.158} & \grlow{-0.045} & \grlow{-0.030} & \grhigh{0.190} & \grlow{-0.093} & \grlow{-0.309} & \grhigh{0.242} & \textbf{\grlow{-0.005}} \\

\cdashline{1-14}

\multirow{5}{*}{\textbf{XGen-7B}}                 
& Mean-R & \grhigh{0.304} & \grhigh{0.103} & \grhigh{0.553} & \grhigh{0.201} & \grhigh{0.230} & \grhigh{0.442} & \grlow{-0.028} & \grhigh{0.350} & \grhigh{0.333} & \grlow{-0.092} & \grhigh{0.418} & \grhigh{0.433} & \textbf{\grhigh{0.271}} \\ 
& BS     & \grhigh{0.042} & \grlow{-0.134} & \grhigh{0.294} & \grhigh{0.011} & \grlow{-0.160} & \grlow{-0.036} & \grlow{-0.090} & \grlow{-0.147} & \grlow{-0.026} & \grlow{-0.285} & \grlow{-0.131} & \grhigh{0.044} & \textbf{\grlow{-0.052}} \\
% & MS     & \grhigh{0.190} & \grhigh{0.091} & \grhigh{0.647} & \grhigh{0.327} & \grlow{-0.022} & \grhigh{0.271} & \grlow{-0.100} & \grhigh{0.120} & \grhigh{0.195} & \grlow{-0.205} & \grhigh{0.100} & \grhigh{0.287} & \grhigh{0.158} \\
% & BaS    & \grhigh{0.159} & \grlow{-0.056} & \grhigh{0.422} & \grlow{-0.010} & \grhigh{0.134} & \grhigh{0.319} & \grhigh{0.011} & \grhigh{0.151} & \grhigh{0.108} & \grlow{-0.052} & \grhigh{0.343} & \grhigh{0.131} & \grhigh{0.138} \\ 
& SUPERT & \grhigh{0.019} & \grlow{-0.180} & \grlow{-0.119} & \grlow{-0.244} & \grlow{-0.194} & \grlow{-0.146} & \grlow{-0.103} & \grhigh{0.021} & \grhigh{0.117} & \grlow{-0.318} & \grlow{-0.372} & \grhigh{0.074} & \textbf{\grlow{-0.120}} \\ 
& BaS-f & \grhigh{0.102} & \grlow{-0.081} & \grlow{-0.009} & \grhigh{0.223} & \grlow{-0.185} & \grlow{-0.107} & \grlow{-0.065} & \grhigh{0.029} & \grhigh{0.118} & \grlow{-0.222} & \grlow{-0.238} & \grhigh{0.096} & \textbf{\grlow{-0.028}} \\ 
& GPT-3.5 & \grhigh{0.039} & \grlow{-0.107} & \grlow{-0.029} & \grhigh{0.015} & \grlow{-0.065} & \grlow{-0.089} & \grlow{-0.154} & \grlow{-0.049} & \grhigh{0.137} & \grlow{-0.158} & \grlow{-0.182} & \grhigh{0.150} & \textbf{\grlow{-0.041}} \\

\bottomrule

\end{tabular}
}
\caption{\small Spearman correlation coefficient between each LLM's metric, and the reference length (measured in terms of tokens).}
\label{corr_target_length}
\end{table*}

==> Tables/unused_findings.tex <==
\begin{table*}[]
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{l}

\toprule 

\textbf{\emph{RQ1: Where do LLMs take their information from when they summarize?}} \\

$\sbullet$ LLMs mostly take information from the beginning of the source. \\
$\sbullet$ Existing summarization datasets are lead-biased, but  LLMs are significantly more lead-biased than the reference. \vspace{0.5em}\\ 
\textbf{\emph{RQ2: Where do LLMs look at within their context window?}} \\

% $\sbullet$ LLMs attend more to the beginning or the end of their context window. \\

$\sbullet$ LLMs are more likely to re-phrase information from the beginning or (to a lesser extent) the end of their context window. \vspace{0.5em}\\ 

\textbf{\emph{RQ3: Does LLMs summarization performance depend on the position of the information?}} \\

$\sbullet$ LLMs summarization performance is sensitive to the position of salient information in
the context window. \\

$\sbullet$ Reference-based evaluation shows a negative correlation between the position of salient information and performance.\vspace{0.5em}\\ 

\textbf{\emph{Analysis:}} \\

$\sbullet$ Control experiments show a strong U-shape \citep{litm} in summarization: when explicitly prompted to, LLMs are good \\ 
at processing information at the beginning or (to a lesser extent) the end of their input, while the middle is largely ignored. \\

$\sbullet$ \emph{Hierarchical} and \emph{incremental} inference can alleviate the middle-curse on scientific paper summarization. \\

$\sbullet$ Inferring on more than 4k tokens shows no significant improvement in performance on long-input summarization tasks, \\
questioning the interest of extending the context window of open-source LLMs. \\


\bottomrule

\end{tabular}
}
%\vspace{-0.5em}
\caption{\small Summary of our findings when applying LLMs in zero-shot to abstractive summarization tasks.}
%\vspace{-1.0em}
\label{findings}
\end{table*}

==> Tables/unused_order_multinews.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\resizebox{\columnwidth}{!}{
\begin{tabular}{llccccc}

\toprule 

\textbf{Model}              
& \textbf{Docs. ordering} 
& \textbf{Mean-R} 
& \textbf{BS} 
& \textbf{SP} 
& \textbf{BaS-f} 
& \textbf{GPT-3.5} \\

\midrule 

\multirow{4}{*}{\textbf{LLAMA-2-7B}}
& Default                               & 29.43 & 82.23 & 51.68 & \textbf{-2.34} & \textbf{4.31} \\
& Shuffle - \emph{mean \small (std)}    & 29.45 \small (0.23) & \textbf{82.49} \small (1.02) & 51.76 \small (0.45) & \textbf{-2.34} \small (0.11) & 4.20 \small (0.04) \\
& BS w/ reference ($\downarrow$)        & \textbf{29.80} & 82.39 & \textbf{51.84} & -2.39 & 4.26 \\
& BS w/ reference ($\uparrow$)          & 29.27 & 81.84 & 51.46 & -2.41 & 4.24 \\

\midrule 

\multirow{4}{*}{\textbf{LLAMA-2-13B}}
& Default                               & 30.59 & 85.75 & 53.12 & -2.09 & 4.26 \\
& Shuffle - \emph{mean \small (std)}    & 30.48 \small (0.15) & 85.78 \small (0.07) & 53.22 \small (0.09) & -2.06 \small (0.03) & \textbf{4.33} \small (0.04) \\
& BS w/ reference ($\downarrow$)        & 30.47 & \textbf{85.79} & 53.15 & -2.07 & 4.25 \\
& BS w/ reference ($\uparrow$)          & \textbf{30.62} & 85.77 & \textbf{53.33} & \textbf{-2.05} & 4.32 \\

\midrule 

\multirow{4}{*}{\textbf{XGen-7B}} 
& Default                               & 27.87 & 84.80 & 55.64 & \textbf{-1.70} & \textbf{4.29} \\
& Shuffle - \emph{mean \small (std)}    & 27.97 \small (0.19) & 84.69 \small (0.13) & 55.63 \small (0.05) & -1.95 \small (0.04) & 4.26 \small (0.02) \\
& BS w/ reference ($\downarrow$)        & \textbf{28.58} & \textbf{85.00} & \textbf{55.79} & -1.93 & 4.28 \\
& BS w/ reference ($\uparrow$)          & 27.05 & 84.25 & 55.56 & -1.99 & 4.22 \\

\bottomrule
                            
\end{tabular}
}
\caption{\small Results on MultiNews with several strategies to order source documents. Mean-R is the Mean-ROUGE, BS is BERTScore, SP is SUPERT, BaS-f is BARTScore-faithfulness. We exclude FLAN-UL2 due to its too short context window for this dataset.}
\label{order}
\vspace{-1.0em}
\end{table}
